homotopy.io: a proof assistant for finitely-presented globular $n$-categories

We present the proof assistant homotopy.io for working with finitely-presented semistrict higher categories. The tool runs in the browser with a point-and-click interface, allowing direct manipulation of proof objects via a graphical representation. We describe the user interface and explain how the tool can be used in practice. We also describe the essential subsystems of the tool, including collapse, contraction, expansion, typechecking, and layout, as well as key implementation details including data structure encoding, memoisation, and rendering. These technical innovations have been essential for achieving good performance in a resource-constrained setting.

==> figures/hopf_stylesheet.tex <==
% Colours
%
%\definecolor{generator-0-0-1-pos}{RGB}{0, 0, 0}
\definecolor{generator-0-0-1-pos}{RGB}{56, 150, 211}
\definecolor{generator-0-0-2-pos}{RGB}{89, 167, 218}
%
\definecolor{generator-1-2-0-pos}{RGB}{192, 57, 43}
\definecolor{generator-1-2-1-pos}{RGB}{212, 78, 64}
\definecolor{generator-1-2-2-pos}{RGB}{220, 109, 97}
%
\definecolor{generator-2-3-0-pos}{RGB}{243, 156, 18}
\definecolor{generator-2-3-1-pos}{RGB}{245, 172, 57}
%
\definecolor{generator-3-3-0-pos}{RGB}{243, 156, 18}
\definecolor{generator-3-3-1-pos}{RGB}{245, 172, 57}
%
\definecolor{generator-4-3-0-pos}{RGB}{39, 174, 96}
\definecolor{generator-4-3-1-pos}{RGB}{46, 207, 114}
%
\definecolor{generator-5-3-0-pos}{RGB}{39, 174, 96}
\definecolor{generator-5-3-1-pos}{RGB}{46, 207, 114}
%
\definecolor{generator-6-4-0-pos}{RGB}{0, 0, 0}
\definecolor{generator-7-4-0-pos}{RGB}{0, 0, 0}
\definecolor{generator-8-4-0-pos}{RGB}{0, 0, 0}
\definecolor{generator-9-4-0-pos}{RGB}{0, 0, 0}
\definecolor{generator-9-4-0-neg}{RGB}{122, 122, 122}
%
\definecolor{generator-10-4-0-neg}{RGB}{122, 122, 122}
\definecolor{generator-11-4-0-pos}{RGB}{0, 0, 0}
\definecolor{generator-12-4-0-pos}{RGB}{0, 0, 0}
\definecolor{generator-12-4-0-neg}{RGB}{122, 122, 122}
\definecolor{generator-13-4-0-pos}{RGB}{0, 0, 0}
\definecolor{generator-14-4-0-pos}{RGB}{0, 0, 0}
\definecolor{generator-14-4-0-neg}{RGB}{122, 122, 122}
\definecolor{generator-15-4-0-pos}{RGB}{0, 0, 0}
\definecolor{generator-16-3-0-pos}{RGB}{0, 0, 0}
\definecolor{generator-16-3-1-pos}{RGB}{20, 20, 20}
%
\definecolor{generator-17-4-0-pos}{RGB}{246, 245, 244}
\definecolor{generator-17-4-0-neg}{RGB}{184, 176, 168}
%
\definecolor{generator-18-4-0-pos}{RGB}{246, 245, 244}
\definecolor{generator-19-2-0-pos}{RGB}{142, 68, 173}
%
\definecolor{generator-20-3-0-pos}{RGB}{243, 156, 18}
\definecolor{generator-21-3-0-pos}{RGB}{39, 174, 96}
\definecolor{generator-22-4-0-pos}{RGB}{0, 0, 0}
\definecolor{generator-22-4-0-neg}{RGB}{122, 122, 122}
\definecolor{generator-23-4-0-pos}{RGB}{0, 0, 0}
\definecolor{generator-24-4-0-neg}{RGB}{122, 122, 122}
\definecolor{generator-26-4-0-pos}{RGB}{246, 245, 244}
\definecolor{generator-29-2-0-pos}{RGB}{241, 196, 15}
%
\definecolor{generator-30-3-0-pos}{RGB}{246, 245, 244}
\definecolor{generator-31-4-0-pos}{RGB}{243, 156, 18}
\definecolor{generator-32-3-0-pos}{RGB}{41, 128, 185}
\definecolor{generator-33-4-0-pos}{RGB}{243, 156, 18}
\definecolor{generator-36-3-0-pos}{RGB}{246, 245, 244}
\definecolor{generator-38-3-0-pos}{RGB}{246, 245, 244}
\definecolor{generator-39-4-0-pos}{RGB}{220, 138, 221}
\definecolor{generator-40-3-0-pos}{RGB}{41, 128, 185}
\definecolor{generator-41-4-0-pos}{RGB}{246, 97, 81}
\definecolor{generator-50-4-0-pos}{RGB}{243, 156, 18}
%
